The cooperative game theory foundations of network bargaining games

We study bargaining games between suppliers and manufacturers in a network context. Agents wish to enter into contracts in order to generate surplus which then must be divided among the participants. Potential contracts and their surplus are represented by weighted edges in our bipartite network. Each agent in the market is additionally limited by a capacity representing the number of contracts which he or she may undertake. When all agents are limited to just one contract each, prior research applied natural generalizations of the Nash bargaining solution to the networked setting, defined the new solution concepts of stable and balanced, and characterized the resulting bargaining outcomes. We simplify and generalize these results to a setting in which participants in only one side of the market are limited to one contract each. The heart of our results uses a linear-programming formulation to establish a novel connection between well-studied cooperative game theory concepts (such as core and prekernel) and the solution concepts of stable and balanced defined for the bargaining games. This immediately implies one can take advantage of the results and algorithms in cooperative game theory to reproduce results such as those of Azar et al. [1] and Kleinberg and Tardos [29] and also generalize them to our setting. The cooperative-game-theoretic connection also inspires us to refine our solution space using standard solution concepts from that literature such as nucleolus and lexicographic kernel. The nucleolus is particularly attractive as it is unique, always exists, and is supported by experimental data in the network bargaining literature. Guided by algorithms from cooperative game theory, we show how to compute the nucleolus by pruning and iteratively solving a natural linear-programming formulation.

==> conclusion.tex <==
%\section{Conclusion}
%
%Discuss difficulties in extending nucleolus to non-secretary and all
%of it to non-bipartite.  Other major open questions?  Axiomatize
%nucleolus in networked bargaining terminology?  Perform lab
%experiments to figure out which solution concepts people play in
%practice?

\paragraph{Acknowledgements.}
%
The authors would like to acknowledge \'Eva Tardos for suggesting
possible connections with the cooperative game theory literature.


==> intro.tex <==
%%% VERIFY CITATIONS!!

\section{Introduction}

Common wisdom has it that the whole is more than the sum of the
parts. In more economic terms, this proverb is a translation of the
fact that two cooperative agents are often capable of generating a
surplus that neither could achieve alone.  For example, the owner of
a music studio, together with a music band, can record and sell an
album; a publishing house, together with an author, can print and
sell a book. The proceeds from the album or the book are the surplus
generated by the cooperation of the agents.  {\it Bargaining theory}
asks how agents divide this jointly generated surplus.

In the 1950s, John Nash proposed a solution to this problem for the
special case of two agents~\cite{N50_Nash}.  His solution, known as
the {\it Nash bargaining solution}, is based on the intuition that,
all else being equal, agents will tend to divide the surplus equally.
If things are not equal, i.e., if some agents have better outside
options than others, then the {\it net} surplus will be divided
equally.\footnote{Nash's solution concept is actually defined for a
  slightly more general problem where the feasible contracting region
  need not be linear; in the special case described herein, Nash's
  solution corresponds to other standard notions as well.
  Nonetheless, we adopt the terminology {\it Nash bargaining solution}
  to be consistent with prior work on this topic in the computer
  science literature.} Since Nash's result, various economists and
computer scientists have extended this solution concept to a networked
setting and defined new equilibrium concepts as
well~\cite{CK08,KT08}. In these settings, each agent has a set of
potential contracts, represented by the network.  The ``outside
options'' of the Nash bargaining solution are now endogenous to the
model and generated by the network structure itself.

We propose looking at the network bargaining game through the lens of
{\it cooperative game theory}.\footnote{This was done in the economics
  literature for the matching game described below~\cite{SS72}, but the
  connections we draw between the computer-science-defined notions and
  the cooperative-game-theory notions are novel.}  In a cooperative
game, sets of agents are mapped to values representing the surplus
they alone can generate.  A solution then assigns a payoff to each
agent.  The literature has a rich history exploring various solution
concepts, their axiomatic properties, and their computability.  By
interpreting the network bargaining game in this context, we are able
to leverage the valuable tools and concepts of cooperative game theory
when studying network bargaining.  Not only does this enable us to
reproduce previous results (with arguably little effort) and derive
these previous results for more general models, but more importantly
perhaps, we are introduced to new refined solution concepts such as
{\it nucleolus} and {\it lexicographic kernel}.  These concepts are
often arguably more predictive than those previously studied.

%\vspace{-3mm}
\paragraph{Our Results.}
In most prior work on networked bargaining, researchers assume each
agent can enter {\it at most one} contract, i.e., the set of contracts
form a {\it matching}.\footnote{An exception is the model of
  Chakraborty and Kearns~\cite{CK08} where agents make multiple deals, but
  the utilities are non-linear.}
%
%This corresponds to the idea that each studio or publishing house has
%only enough resources to support {\it one} artist, and each artist has
%only enough stamina to generate {\it one} work at a
%time. 
Additionally, contracts are often assumed to be of equal worth. 
%That
%is, every book or album generates the same amount of surplus,
%regardless of which pair of agents contract to create it. 
%
In this paper, we generalize these models by assigning each agent a
capacity constraint and allowing him or her to participate in a number
of contracts limited by this capacity.
%\footnote{We note that our
%  models cannot be reduced to the matching case by simply creating
%  multiple copies of agents as these copies would then compete with
%  one another.  See Section~\ref{sec:prelim} for further discussion.}
%In other words, a studio may be able to record multiple albums
%simultaneously; an author may be able to work on several books
%simultaneously.  
We also allow contracts to generate varying amounts of surplus.
%
We mainly focus our efforts on the important special case of bipartite
networks, or networks like the music and literature examples above, in
which each agent can be divided into one of two types depending on
which type of agents he or she contracts with. 

The most basic question in these models is to develop predictions
regarding which contracts will form and how much each agent will earn
as a result. A successful prediction should be {\it intuitive}, {\it
  computationally tractable}, and {\it unique}.  
%
To this end, Kleinberg and Tardos~\cite{KT08} proposed a solution
concept for the matching case called {\it stable} and a refinement
called {\it balanced} that are natural generalizations of the Nash
bargaining solution for the two-player case~\cite{N50_Nash}.

We first show how to characterize all stable solutions in our general
setting using a linear-programming formulation which is a
generalization of one developed by Shapley and Shubik~\cite{SS72} for
the matching case.
%
We then introduce a special case of our problem in which one side of
the market is severely capacity-constrained.  In particular, we assume
agents on one side of the market can enter into {\it at most one}
contract each while the other side has general constraints.  
%This
%models situations in which, for example, a music studio or publishing
%house can produce multiple works of art simultaneously, but each
%artist can only produce one work of art at a time. 
In this constrained setting, we draw connections between balanced and
stable outcomes and the cooperative-game-theoretic notions of {\it
  core} and {\it prekernel}.  These notions look for solutions that
are stable with respect to deviating coalitions of any size.  Unlike
the general setting, we prove that the set of stable
solutions and the core coincide in this setting, as do the set of balanced solutions
and the prekernel.  This result is of particular interest as the core
and prekernel are axiomatic solution concepts of exponential
description size (essentially they require that certain conditions
hold for {\it every} subset of agents), whereas the notions of stable
and balanced solutions have inherently polynomial descriptions.
%
\iffalse
Hence while it is significantly more believable that agents will find
stable/balanced solutions (there are only polynomially many conditions
they must check), our result shows that for this particular game they
also find the intuitively natural core/prekernel.  In essence,
deviating coalitions of size more than two are irrelevant for our
game.  
\fi
%
These connections allow us to leverage existing results in the
cooperative game theory literature (such as those for computation of
core, prekernel, nucleolus, and lexicographic kernel) to motivate and
derive solutions in our setting.  

As for leveraging tools from cooperative game theory, the connections
we draw imply that the techniques of Faigle, Kern, and
Kuipers~\cite{FKK98_NucKer} for finding a point in the prekernel of a
game can be adapted to find a balanced solution for our constrained
bargaining game.  Indeed, the resulting algorithm as well as its
analysis is essentially the same as the local dynamics given in Azar
et al.~\cite{ABCDP09}.
%
These connections also have implications for the model of Kleinberg
and Tardos~\cite{KT08}.  In their model, the set of possible contracts
is not necessarily bipartite, but instead each agent is restricted to
participate in at most one contract.  Our aforementioned results
regarding stable and balanced solutions can be adapted to this
setting.  Since the set of stable solutions and core coincide, we are
able to characterize all graphs which have at least one stable
outcome.  Namely, a graph has a stable outcome if and only if the
simple maximum-weight matching LP relaxation has integrality gap
one. Since the set of balanced solutions and the prekernel coincide,
we can obtain the Kleinberg-Tardos result for constructing a balanced
outcome in polynomial time using simple and well-known results from
the economics literature rather than combinatorial constructs such as
posets and Edmonds-Gallai decompositions.

Perhaps more importantly, this connection to cooperative game theory
guides us in our search for solution concepts for our game.  The set
of stable/balanced and core/kernel solutions previously proposed may
be quite large and hence not terribly predictive.  With the goal of
computing a unique and predictive outcome for our game, we propose and
motivate the cooperative-game-theoretic notion of {\it nucleolus} as
the ``right'' outcome.  The nucleolus is unique and symmetric in that
agents with similar opportunities have similar earnings.  It is also
supported by economic experiments, as discussed in
Section~\ref{sec:nucleolus}.  Additionally, for the above model, we
show that the nucleolus is computationally tractable.  We prove this
by following an iterative linear-programming-based approach used
previously by
economists~\cite{GMOZ96_Nuc,FKFH98_Nuc,SR94_Nuc,FKK98_NucKer} and
computer scientists~\cite{DFS06} in unrelated contexts.  In order to
adopt this approach to our setting, we show how to prune the linear
programs, creating programs of polynomial size. The main technical
difficulty is to prove that this pruning maintains the essential
relationships between the iterated linear programs and thus still
computes the nucleolus.

%\vspace{-3mm}
\paragraph{Related work.}  
The most closely related work to ours is that of Kleinberg and
Tardos~\cite{KT08}.  That paper defines stable and balanced solutions
for the matching case mentioned above.  They then give an efficient
characterization of stable/balanced solutions based on posets and the
Edmonds-Gallai decomposition.  Our work re-derives and generalizes some
of their results using simple and well-known results from the
economics literature.
%
Very recently, Azar et al.~\cite{ABCDP09} show that local dynamics
does in fact converge to a stable and balanced solution.
Incidentally, the connection that we establish between the solution
concepts of prekernel and balanced would immediately imply the same
local algorithm via a former result of Stearns~\cite{Stearns}; see
Section~\ref{sec:focs-result} for more details.  
We also learned of two other very recent results:
Kanoria et al.~\cite{KBBCM09}  addresses the problem of finding a ``natural'' 
local dynamics for this game,
and Azar, Devanur, Jain, and Rabani~\cite{ADJR10} also study a special
case of our problem through cooperative game theory and propose
nucleolus as a plausible outcome of the networked bargaining game.
%
The work of Chakraborty et al.~\cite{CKK09} as well as that of
Chakraborty and Kearns~\cite{CK08} considers a related problem, in
which there is no capacity constraints on the vertices but agents have
non-linear utilities.  They explore the existence and computability of
the Nash bargaining solution as well as the proportional bargaining
solution in their setting.
 
Much recent literature has focused on the computability of various
solution concepts in the economics literature.  In the noncooperative
game theoretic setting, the complexity of Nash and approximate Nash
equilibria has a rich recent
history~\cite{TS07,KS07,KPS06,DMP06,DMP07,CD06,CDT06,BBM07,DP09}.  In
cooperative-game-theoretic settings, the core of a game defined by a
combinatorial optimization problem is fundamentally related to the
integrality gap of a natural linear program, as observed in numerous
prior work~\cite{Bondareva,Shapley67,JV01,MS03,IMM05}.  The
computability of the nucleolus has also been studied for some special
games~\cite{DFS06,KP03_Nuc,SR94_Nuc,FKK98_NucKer,FKK99_Nuc,FKK98_Comp,GMOZ96_Nuc}.

Much of our work leverages existing results in the cooperative game
theory literature; these results will be cited as they are used.

